180-degree Outpainting from a Single Image

Presenting context images to a viewer's peripheral vision is one of the most effective techniques to enhance immersive visual experiences. However, most images only present a narrow view, since the field-of-view (FoV) of standard cameras is small. To overcome this limitation, we propose a deep learning approach that learns to predict a 180{\deg} panoramic image from a narrow-view image. Specifically, we design a foveated framework that applies different strategies on near-periphery and mid-periphery regions. Two networks are trained separately, and then are employed jointly to sequentially perform narrow-to-90{\deg} generation and 90{\deg}-to-180{\deg} generation. The generated outputs are then fused with their aligned inputs to produce expanded equirectangular images for viewing. Our experimental results show that single-view-to-panoramic image generation using deep learning is both feasible and promising.

==> PSNR_NRMSE.tex <==
% !TEX root = ../TPAMI19SI.tex

\begin{table*}[tbh]
\centering
\caption{Average image quality scores among subjects for different categories and outpainting methods.}
\begin{tabular}{@{}lllllll@{}}
\toprule
Method     & mountain & street & field & lobby\_atrium & church & restaurant \\ \midrule
ExtVision                        & 68.40          & 58.90          & 73.75          & 52.95                                                  & 55.45          & 50.00          \\ 
ExtVision w/ our blending method & 70.65          & \textbf{61.05}          & 78.05          & 55.15                                                  & 57.30          & 54.00          \\
Ours (90\degree)                        & \textbf{77.05} & {60.35} & \textbf{79.30} & \textbf{65.80}                                         & \textbf{61.80} & \textbf{58.55} \\
\hline
AmbiLux TV                       & 72.45          & 60.25          & 71.60          & 53.85                                                  & 54.20          & 58.60          \\
Ours (180\degree)                       & \textbf{81.65} & \textbf{61.25} & \textbf{83.20} & \textbf{68.60}                                         & \textbf{65.35} & \textbf{61.85} \\
\bottomrule
\end{tabular}
\label{tbl:human_study}
\end{table*}

\begin{table*}[tbh]
\centering
\caption{PSNR and NRMSE for different categories and outpainting methods (narrow to 90\degree sub task).}
\begin{tabular}{c|c|ccc|ccc}
\hline
\multirow{2}{*}{Critera} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{Indoor categories}     & \multicolumn{3}{c}{Outdoor categories}             \\ \cline{3-8} 
                         &                        & lobby\_atrium   & church & restaurant      & mountain        & street          & field           \\ \hline
\multirow{2}{*}{NRMSE}   & ExtVision              & 0.390           &  \textbf{0.397}   & 0.496           & 0.263           & \textbf{0.369}  & 0.243           \\
                         & Ours                   & \textbf{0.373}  &  0.409 & \textbf{0.435}  & \textbf{0.251}  & 0.378           & \textbf{0.237}  \\ \hline
\multirow{2}{*}{PSNR}    & ExtVision              & 15.183          &  
\textbf{16.157} & 13.608          & 16.642          & \textbf{15.334} & 17.973          \\
                         & Ours                   & \textbf{15.609} &   15.947  & \textbf{14.754} & \textbf{17.295} & 15.214          & \textbf{18.486} \\ \hline
\end{tabular}
\label{tbl:to90}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tbh]
\centering
\caption{PSNR and NRMSE for different categories and outpainting methods (90\degree to 180\degree sub task).}
\begin{tabular}{c|c|ccc|ccc}
\hline
\multirow{2}{*}{Critera} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{Indoor categories}              & \multicolumn{3}{c}{Outdoor categories}             \\ \cline{3-8} 
                         &                        & lobby\_atrium   & church          & restaurant      & mountain        & street          & field           \\ \hline
\multirow{2}{*}{NRMSE}   & AmbiLux                & 0.437           & 0.506           & 0.526           & 0.332           & 0.423           & 0.300           \\
                         & Ours                   & \textbf{0.417}  & \textbf{0.459}  & \textbf{0.458}  & \textbf{0.318}  & \textbf{0.398}  & \textbf{0.293}  \\ \hline
\multirow{2}{*}{PSNR}    & AmbiLux                & 13.901          & 14.353          & 13.275          & 14.761          & 13.561          & 16.416          \\
                         & Ours                   & \textbf{14.524} & \textbf{15.158} & \textbf{14.505} & \textbf{14.883} & \textbf{14.160} & \textbf{16.577} \\ \hline
\end{tabular}
\label{tbl:90to180}
\end{table*}

==> ablation_studies.tex <==
% !TEX root = ../TPAMI19SI.tex
\begin{table*}[bth]
\centering
\caption{PSNR and NRMSE for different generator architectures.}
\begin{tabular}{c|c|ccc|ccc}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{Category}} & \multicolumn{1}{l|}{\multirow{2}{*}{Critera}} & \multicolumn{3}{c|}{Near periphery generation}      & \multicolumn{3}{c}{Mid periphery generation}        \\ \cline{3-8} 
\multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                         & ResNet\_6blocks & ResNet\_9blocks & U-Net           & ResNet\_6blocks & ResNet\_9blocks & U-Net           \\ \hline
\multirow{2}{*}{lobby atrium}                  & NRMSE                                         & 0.416           & 0.426           & \textbf{0.373}  & 0.438           & 0.457           & \textbf{0.417}  \\
                                               & PSNR                                          & 14.642          & 14.453          & \textbf{15.609} & 13.901          & 13.765          & \textbf{14.524} \\ \hline
\multirow{2}{*}{mountain}                      & NRMSE                                         & 0.283           & 0.280           & \textbf{0.251}  & 0.315           & 0.329           & \textbf{0.318}  \\
                                               & PSNR                                          & 16.104          & 16.325          & \textbf{17.295} & \textbf{15.020 }         & 14.581          & 14.883 \\ \hline
\end{tabular}
\label{tbl:resnet_vs_unet}
\end{table*}

==> fig_halo.tex <==
\begin{figure}
\centering

% \begin{subfigure}[b]{.4\textwidth}
% \centering
% \includegraphics[width=.4\textwidth]{example-image}\quad
% \includegraphics[width=.4\textwidth]{example-image}

% \caption{}
% \end{subfigure}\quad
% \begin{subfigure}[b]{.4\textwidth}
% \centering
% \includegraphics[width=.4\textwidth]{example-image}\quad
% \includegraphics[width=.4\textwidth]{example-image}

% \caption{}
% \end{subfigure}
\centerline{
\includegraphics[height=2cm]{halo/dustroad_256x256_fake_context.png}
\includegraphics[height=2cm]{halo/Places365_val_00000041_fake_B.png}
\includegraphics[height=2cm]{halo/Places365_val_00000941_fake_B.png}
\includegraphics[height=2cm]{halo/Places365_val_00005112_fake_B.png}
}
% \centerline{
% }
\caption{Halo artifacts when padding the input.}
\label{fig:halo}
\end{figure}

==> fig_more_results.tex <==
\begin{figure*}[tbh]
\centerline{\includegraphics[height=4.8cm]{demo.jpg}} % 5cm
%  \vspace{2.0cm}
\caption{More results on diverse scenes. The first row shows the input images, while the next row shows the outputs generated using our method. Images are from the test set, i.e. the \texttt{others} category of the SUN360 dataset.
\ctext[RGB]{204, 255, 0}{Projection was applied to allow viewing panoramic images in a normal field of view.}
}
\label{fig:demo}
\end{figure*}

\begin{figure*}[bht]
\centerline{\includegraphics[width=18.3cm]{comparison.jpg}} % 18.5cm
%  \vspace{2.0cm}
{ \hfill Input \hfill ExtVision~\cite{kimura2018extvision} \hfill Multiscale~\cite{aides2011multiscale} \hfill Ours (90\degree FoV) \hfill  Ours (180\degree FoV) }
\caption{Comparison with other algorithms. Our method is shown in the far right image.
\ctext[RGB]{204, 255, 0}{Projection was applied to allow viewing panoramic images in a normal field of view.}
}
\label{fig:comparison}
\end{figure*}

==> fig_single_cat_results.tex <==
\begin{figure*}[bth]
\centerline{\includegraphics[height=17.0cm]{val.png}} %18.1cm for pami
\caption{
Single-category results. 
The networks were trained and tested on three outdoor categories (mountain, street and field) and three indoor categories (lobby atrium, church and restaurant). Each row shows a sample of the held-out images in the validation set of a category. From left to right: the padded input images, the 90\degree ~images generated from the inputs, the ground truth 90\degree images, the 180\degree images generated from the ground truth 90\degree ~images and the ground truth 180\degree ~images.
}
\vspace{-0.2cm}
\label{fig:res_outdoor}
\end{figure*}

==> human_study.tex <==
% !TEX root = ../TPAMI19SI.tex
\subsection{Human Study}

We conducted a human study to investigate the quality of experience (QoE) of panoramic images generated by our method.   
% There is currently no defined protocol to evaluate QoE for a single-view-to-panoramic image generation system
The generated images were displayed on a HTC Vive VR headset
% Image playback was supported by 
back-ended with
a dedicated high performance server (Intel i7-6700, 32GB memory, NVIDIA TITAN X). % 1TB hard drive, 
The interface of the subjective test was built using Unity Game Engine. 
In the following subsections, we will explain how the images were rated and the detailed protocol of the human study.

\subsubsection{Image Quality Scoring}
We recruited 20 students at The University of Texas at Austin, 
including 7 females and 13 males. 
% Each subject was informed briefed about the goals of the study and presented with the detailed procedure in written form. 
% A consent form was also signed by the subject. 
Each subject was asked to view a randomized series of panoramic images,
and to rate each image with regards to the quality of their viewing experiences, while trying not to be affected by the degree of appeal of the content.
% so that the generated periphery regions viewed by central vision. 
% only, without looking around. 
We followed the Single Stimulus Continuous Quality evaluation methodology described in recommendation ITU-R BT 500.13~\cite{series2012methodology}
% ~\cite{series2012methodology},
% ~\cite{series2012methodology}, 
% I. T. Union, “Methodology for the subjective assessment of the quality of television pictures ITU-R recommendation BT.500-13,” Tech. Rep.,2012.
using a continuous rating scale from 0 to 100, where 0 indicates the worst quality.

% The subjects were asked whether they were prone to dizziness when participating in either a VR or 3D environment beforehand, to eliminate subjects who were not suitable for this subjective study. 
% The visual acuity of each subject was determined using the Snellen test, and each subject was asked to wear their corrective lenses to achieve normal vision when participating in the study.
% (No stereo vision but simply put on a sphere) Each subject also participated in a RanDot Stereo test of their stereo vision and depth perception. 
% The range of Interpupillary Distances (IPD) of the HTC Vive is 60.3mm-73.7mm. For those subjects whose IPD was outside of this range, a period of experimentation with the HMD was allowed. If the subject felt uncomfortable, then it was recommended that he/she not perform the test.



% Since wearing a VR helmet for a long period of time can
% lead to feelings of fatigue and dizziness, each viewing session
% was limited to a duration of 30 minutes and the subjects were
% free to take a rest if they felt any discomfort. 

% If any test showed impairment, the subject was recommended not to take this test, but if the subject decided to perform the test, the results were discarded.

% \subsection{Session Design}
To limit each subject's viewing time, 
the quality rating bar appeared after 5 seconds of viewing each image.
% a gray canvas displayed as background of the rating bar
% , as shown in Figure 8. 
% The quality scale was in the center of the subject’s field of view, wherever he moved his head. 
Five Likert labels (Bad, Poor, Fair, Good, Excellent) marked the rating bar to help guide the subject when making ratings. 

% To rate the images, the subjects used the hand controllers supplied with the VR headset to choose the desired score on the quality scale. After the subject was satisfied with the score chosen, he or she clicked on ’Submit and Next’ to see the next image. Once the subject submitted the score, the name and score of the image were written to file.

\subsubsection{Session Design}
Each subject participated in two sessions separated by
at least 24 hours, to avoid fatigue.
% To avoid boredom and fatigue to adversely affect results,
% each session was kept under 30 min as in ITU recommendations~\cite{itu2007methodology}.
In each session, panoramic images from 6 categories (3 outdoor
categories: mountain, street and field; 3 indoor categories: lobby atrium, church and restaurant) were randomly selected. 
% The "hidden" reference image was included in each session. 
We randomly picked 3 input images from the test set of each category, and applied different methods to obtain panoramic images for rating. To reduce the effects of visual memory comparisons, images having the same content were separated by at least 3 images of different content.
% The average viewing time for each session was 27 minutes, with the average viewing and rating time for each image being around 23 seconds.

\textbf{Session I: Comparison of 90\degree~outpainting methods.}
In this session, the FoV was fixed to 90\degree. This allowed the subjects to judge the quality of images generated both by ExtVision and by our method. 
We also implemented and compared ExtVision modified with our blending method to allow for fair comparison only on generated content. Those areas outside of 90\degree~FoV were rendered as black. 

\textbf{Session II: Comparison of 180\degree~outpainting methods.}
Since ExtVision cannot perform 180\degree~outpainting, we could only compare our method against the AmbiLux TV method. To simulate AmbiLux TV, we obtained the 180\degree~panoramic images by resizing the input image.

\subsubsection{Results}

The subjective test results are reported in Table~\ref{tbl:human_study}.
Our method delivered the highest subjective quality scores among most categories, often by significant margins. 
We also computed and report the NRMSE and PSNR as references.
% Although the output of the generator is best evalu-
% ated qualitatively, we still utilize RMSE as our primary
% quantitative metric. 
The quantitative metric results for narrow-to-90\degree image generation and 90\degree-to-180\degree generation are given in Tables~\ref{tbl:to90} and~\ref{tbl:90to180}, respectively.
Both qualitative and quantitative evaluation show that our method tends to produce more appealing results than existing methods.

We observed that the outpainting task is more challenging on some categories than  on others. It is harder to train on a complex, spatially diverse scene (such as the crowded interior of a restaurant) than on a scene containing redundant patterns or textures (such as a field).
By comparing the scores reported on two tasks (\cf Tables~\ref{tbl:to90} and~\ref{tbl:90to180}), it is apparent that the second task is more challenging. This makes sense, since the second task involves both image outpainting, as well as geometric transformation.

% Given a ground truth image I tr ∈
% [0, 255] 128×128×3 and a normalized generator output image
% I o 0 = 255 · I o ∈ [0, 255] 128×128×3 , we define the RMSE as:





==> main_body.tex <==
% !TEX root = ../outpaint.tex
% "\def\mode{%2}\input{%1.tex}"
% \section{Introduction}

% \hspace{2cm}
% \IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}


\section{Introduction}\label{sec:introduction}
\label{sec:intro}

% \renewenvironment{mdframed}[1]{}


% On the one hand, VR is hot
% First introduce 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Today, movie theaters and TV screens fill only a limited part of a user’s field of view due to limited screen sizes and image formats. 
% Image resolution defines the optimal distance from the screen for a good viewing experience based on the viewer’s visual acuity. 
% This calculation then leads to a given field of view occupied by the projected image, depending on the screen size, i.e., from 36 degree at the back of a movie theater to 90 degree in the front. 
% These figures are based on the guidelines created in 1994 by the Society of Motion Picture and Television Engineer (SMPTE), which recommended that the screen delimit a minimum horizontal angle of 30 degree for viewers in the back of the room, the optimal angle probably being approximately 50 degree [1]. This corresponds to a distance of 3.45 Picture Heights, using the contemporary picture proportions of 1.85:1 for the movie theater.

% When a viewer’s entire field of view is filled, it creates a
% more immersive experience, increasing their enjoyment of the content. Research has therefore been conducted into
% extending the content to outside the front screen. Several methods may be used for this, the first consisting of captur- ing additional content with a wide field of view [2],
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Cinemas provide a more immersive experience compared with normal televisions by presenting a bigger field-of-view (FoV) to fill a viewer’s peripheral vision.
% However, most images/videos today only present a narrow-angle view since the FoV of standard cameras is very small.

% \myadded{1}{test add some thing v1}
% \myadded{2}{test add some thing v2}
% \myadded{3}{test add some thing v3}

\IEEEPARstart{A}{lthough} image inpainting has been widely studied,
its cousin, image outpainting, has been relatively unexplored~\cite{sabini2018painting}.
% Unlike Image Inpainting which aims to replace a relatively small portion of missing or corrupted parts in the interiors of images,
% Image Outpainting extends the exterior of images by predicting a relatively big portion of 
Image inpainting algorithms aim to predict relatively small missing or corrupted parts of the interiors of images, based on evidence from surrounding pixels. Ultimately, it may be viewed as a problem of interpolation.
By contrast, image outpainting is to extend images beyond their borders, thereby creating larger images with added peripheries.
Strictly speaking, this is an extrapolation problem. However,
the goal may be to extrapolate a rather large periphery, containing objects and context. 
% are different to extrapolate by simply numerically extrapolating. 
% where often, a large portion of exteriors needs to be predicted from less neighboring information. 
% the surrounding 
 % where often, only small regions of the image are affected.
Since those two research fields are closely related but slightly different,
image inpainting techniques 
can be borrowed, with some modifications,
% taking account to their differences
to repurpose them for image outpainting tasks.

% \IEEEPARstart{O}{ne}
% Image outpainting techniques have different application environments than do image inpainting.
The most common application of image outpainting 
% is context generation for video extrapolation.
is to generate context for immersive video extrapolation.
% video expansion and texture creation.
By generating peripheral context images to expand the size of an original video content~\cite{jones2013illumiroom},
a viewer's field of view may be greatly expanded, thereby creating a more immersive, vivid, and realistic experience~\cite{turban2017extrafoveal}.
Although peripheral presentation systems have been constructed~\cite{jones2013illumiroom,avraham2011ultrawide,aides2011multiscale,kimura2018extvision}, 
they are not yet very popular because of the difficulty of creating the peripheral context images. 
% Recent years have seen significant efforts applied to the development of 
% Presentation of images to a viewer’s peripheral vision makes the experience of watching a video more immersive and exciting. 
% \myreplaced{2}{
Here we attack this problem by employing deep neural networks (DNNs).
Unlike existing systems that only extend input images horizontally and vertically by a limited extent, 
% our methods covers a FoV of 180 degree.
we more ambitiously generate 180\degree panoramic context-images, which if successful, could be used to significantly deepen immersive visual experiences,
as exemplified in Fig.~\ref{fig:intro}.
% }{Fortunately, a recent work~\cite{kimura2018extvision} has shown a break-through to this problem by utilizing deep neural networks (DNNs). 
% % Recently, ExtVision~\cite{kimura2018extvision} applied deep neural networks (DNNs) to this task and achieved visual pleasing results. 
% They also conducted a human study to prove that the peripherally projected images generated by their system named ExtVision are sufficient for a positive enhancement of visual experiences.
% % Based on pix2pix~\cite{pix2pix2017}, they build a system called ExtVision  and present visual pleasant results.
% In this paper, we further improve the visual experiences by proposing a single-view to panoramic generation method.
% As shown in Fig.~\ref{fig:intro}, unlike ExtVision that only extends the input images horizontally and vertically to some extent, our methods covers a FoV of 180 degree.}
To the best of our knowledge, 
this is the first such method to be attempted. 
% is proposed
% it is the first time DNNs has been applied for this task.

\begin{figure}[htb]
\centerline{\includegraphics[width=8.5cm]{intro.png}}
%  \vspace{2.0cm}
\caption{Left: a single-view image. Right: a 180-degree panoramic image generated from the left single-view image.}
\label{fig:intro}
\end{figure}

\begin{figure*}[t]
\centerline{ % height=6.6cm
\includegraphics[height=6.4cm]{existing-system.png}
}
\vspace{-0.5cm}
\caption{Existing peripheral presentation systems.
Ambilight TV \textcopyright 2011, Siberex /
% material from the Wikipedia article 
\url{https://commons.wikimedia.org/wiki/File:Ambilight-2.jpg}.
% , which is released under the <a href="https://creativecommons.org/licenses/by-sa/3.0/">Creative Commons Attribution-Share-Alike License 3.0</a>.
AmbiLux TV \textcopyright
2015, Michael Rathmayr/ 
% \url{https://mashable.com/2015/09/03/philips-ambilux-projector-tv/#qB8u_H.pKiqJ}.
\url{https://mashable.com/2015/09/03/philips-ambilux-projector-tv/}.
Other images are from the corresponding papers.
}
\label{fig:systems}
\end{figure*} 


Single-view-to-panoramic generation is a highly ill-posed inverse problem, since there are infinitely many possible panoramic images that may correspond to a single-view image under essentially any match criterion. 
One way that we seek to constrain the task is by taking into account properties of peripheral visual perception.
% human visual system (HVS).
First, we exploit the observation that generating high resolution panoramic images is not necessary, since human peripheral vision is lower in spatial resolution than in the central visual field.
Because of this, foveated rendering techniques~\cite{patney2016foveated,guenter2012foveated} 
can be used to
unlock significant speedups by dividing the image 
% destined for the headset’s display 
that is to be displayed %on a 
into multiple sections of varying resolution. 
% employing a multi-resolution 
Our method uses a foveated framework, both to reduce the computation time and to accelerate network training.
% Foveated rendering synthesizes images with progressively less detail
% outside the eye fixation region, potentially unlocking significant
% speedups for wide field-of-view displays, such as head mounted
% displays, where target framerate and resolution is increasing faster
% than the performance of traditional real-time renderers.
%
% Oculus’ FFR technology sub-divides the image destined for the headset’s display into 19 sections of varying resolution. 
% Therefore, increasing the resolution of panoramic images only bring a lot of computation burden without augmenting visual experiences. 
% and accurate 
% and visual acuity 
In our approach, we allow for a degree of inaccurate or unrealistic image generation in the periphery, because 
when the image is appropriately viewed, \eg, with a VR device,
then the distortions may be designed to be less conspicuous, or even unseen by exploiting the decreased visual acuity in the peripheral visual field~\cite{thibos1987retinal}, as well as
% there is a loss of visual acuity with increasing distance from the fovea, 
% The 
visual crowding~\cite{lettvin1976seeing}.
Crowding is a phenomenon whereby peripheral vision is not only blurred relative to foveal vision, but may also be perceived as normal even if the peripheral content is otherwise distorted~\cite{rosenholtz2012rethinking,fridman2017sideeye,fridman2017fast}.
% Fig. presents a simulation generated by ....
If properly designed, context images can provide an adequate representation of peripheral vision even if the generated periphery is somewhat distorted. 

Just as DNN-based methods have achieved considerable success on solving the image inpainting problem, 
we build on these concepts, with important modifications,
% the existing completion networks 
to implement the challenging single-view-to-panoramic image generation task.

% not limit to this perticular application
% While our explorations are performed in the context of interactive
% games, the same or similar illusions could be used
% to enhance movies and television content. 

% movies and television content. 



We make the following contributions:
\setlist{nolistsep}
\begin{itemize}[noitemsep] % ,leftmargin=*
	% \itemsep0em
	\item[--] We derive a recommended input field of view and output resolution when generating single-view-to-panoramic images. % generation 
	\item[--] We design a two-stage foveated framework by which to efficiently spatially extend the image content.
	\item[--] We use DNNs to generate peripheral image content.
	 % and traditional 
	\item[--] Because our method does not seek to minimize a boundary error functional, visible boundary effects can occur. To ameliorate this, we deploy a simple blending method to fuse the generated content with the original content along the image boundaries.
	\item[--] We analyze the experimental results, discuss the limitations of our approach, and consider future work.
	% A DNN-based method using the proposed framework.
	%generate an 180-degree panoramic image from a single-view image.
\end{itemize}
% and description of the proof-of-concept single system 
% for real-time generation of peripheral projected illusions
% discovery of the limitations of our method
% • Implementation of 11 illusions that demonstrate the
% important dimensions of the design space
% • Analysis of the design space of peripheral projected illusions
% • Discussion and implementation of methods to drive illusions
% from new and existing content
% • Feedback from 10 casual gamers and 15 expert game
% designers over two separate evaluations; showing the
% most promising dimensions of the design space 
 % (a special rig of multiple cameras or a dedicated camera), not to mention the challenges of video capturing and stitching in some special sceneries.
% received a lot of attention.
% More recently, the development of consumer level heads-up
% Virtual Reality (VR) devices has created interest in a new generation
% of user interaction and user experiences. 
% the rise of consumer level heads-up displays for virtual reality.
% However, we cannot experience 360 based on traditional normal view content.
% What if we can 

 % and various applications such as artistic photo editing and image-based lighting with HDR environment maps. 

% \section{Related Work}
% \label{sec:relatedWork}

% #############################################################################
% \section{Related Work}
% \label{sec:relatedWork}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % If the context-image already exists, such as in games, PC work, and movies filmed with dedicated context-capturing equipment, we do not need to create it [3, 10]. 
% % However, in the case of existing legacy content or content shot without dedicated equipment, it is necessary to estimate and generate context-images only from video data. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textbf{traditional methods}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% ~\cite{jones2013illumiroom}.
% Philips’s AmbilightTV [22] is the simplest implementation for creating context-images. The TV has a series of color LED strips on its edges, and the colors of the LEDs dynamically change to match television contents. In a follow-up project, Philips created AmibLuxTV [22] which projects an enlarged image of the television on the wall by a projector attached to the back of the television. Infinity-By-Nine [12] is a CAVE [4] -like system with three projectors and screens around a television. The context-image is generated by their method using optical flow, color analysis, and heuristics. Aides, et al. [1] applied the PatchMatch algorithm developed from an original work by Avraham and Schechner [2] to the extrapolation video to an image’s peripheral area. Although the videos generated by this method seem very natural depending on the scene, it takes a few minutes of processing time per frame. Turban, et al. [16] developed a lighter algorithm than the PatchMatch algorithm, but the generated images are much more artificial than those generated by PatchMatch. As described above, methods have not yet been proposed for generating sufficient context-images with respect to processing speed and naturalness.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Deep generation methods}

% ExtVision
% ####################################################################


% the peripheral vision  
% However, in wide FoV displays such as VR, 96\% of pixels are outside this \ang{20} boundary [31].


% In order to appropriately extend the content around the screen, a full understanding of human vision capacities and characteristics is necessary, allowing us to know what a viewer can and cannot see in the extended content, what the eye is sensitive to, and therefore what could distract the viewer from the main content. 

% The area of human vision in which we are particularly interested here is peripheral vision: how the human eye perceives the content it is not focused on, how much detail it can perceive in luminance, color or motion, and what could be potentially distracting, forcing users to turn their heads and therefore hindering their experience. All these factors are considered whilst keeping in mind that 

% apply our algorithm to only the center of the image.
% only require statisti
% any panoramic images that are consistent with 
% ; therefore,
% Traditional video extrapolation methods use patch-matching and 
% One may ask how it is possible to complete the missing surrounding information only based on a narrow-angle central view. 
% In particular, our work divide the problem into to sub problems:

% \subsection{Immersive Displays/peripheral presentation systems}
% \subsection{Context-image Generation and Image Completion}

% \myadded{2}{}


\section{Related Work}
\label{sec:relatedWork}


% \subsection{Context Image Generation}
\subsection{Peripheral Presentation Systems}
% \subsection{Immersive Displays}

Fig.~\ref{fig:systems} depicts some existing peripheral context generation systems
which we can conveniently divide into three categories,
each of which we
% As shown in Fig.~\ref{fig:systems}, 
% we divide existing systems into three categories
briefly review in the following.
% In this section, we briefly review the existing peripheral presentation systems.

% \subsubsection{CAVE-like Systems}

% \subsubsection{Traditional Methods}
% \textit{Ambilight Systems.}
\textit{Image-Plane-Extension Systems.}
%A first rough step in this direction is the Ambilight television system [16]. There, the wall around the television screen is illuminated in real-time with light that matches the colors that exist at the margins of each frame. Related setups are discussed in [7] and [18].
% Philips TV. Experience Ambilight | Philips. Retrieved
% January 9, 2018 from https://www.philips.co.uk/c-m-
% so/televisions/p/ambilight
% Philips-Ambilight. Philips has unveiled ’ambilight technology’ for TVs.http://www.televisionpoint.com/news/newsfullstory.php?id=1124298851. 1
% This concept was commercialized to some degree by Philips with their Ambilight TV [35].
%%%%%%%%%%%%%%%%%%%%%%%
% Ambilight TV systems
%%%%%%%%%%%%%%%%%%%%%%
% The set’s svelteness is further emphasised by both the strikingly minimalist feet attached beneath the bottom corners of the TV, which are angled so that you see only their narrow edge, and a four-sided implementation of Philips’ Ambilight technology.
% For those unfamiliar with Ambilight, it’s a system that uses LED lights on the TV’s rear to throw out coloured light that can be set to match the colour content of the images you’re watching. It achieves this with startling colour and positional accuracy.
% Most Ambilight implementations I’ve seen recently only involve the left and right sides of the screen, but the 55PUS8601’s four-sided approach makes the immersive effects of the technology even more impressive.
%
% * The simplest implementation for creating context-images
This concept of peripheral presentation was successfully commercialized to some degree by Philips in the form of the Ambilight TV~\cite{weffers2011immersive}
% Philips's AmbilightTV~\cite{weffers2011immersive} 
% Ambilight TV 
 which uses LED lights on the TV's rear to throw out colored light that dynamically changes to match the displayed television content. 
% that can be set to match the color content of the images. 
% Using a series of color LED strips on its edges, 
% the colors of the LEDs dynamically change to match television contents. 
% uses LED lights on the TV’s rear to throw out colored light that can be set to match the color content of the images. 
% Most Ambilight implementations I’ve seen recently only involve the left and right sides of the screen, but the 55PUS8601’s four-sided approach makes the immersive effects of the technology even more impressive.
% Philips Ambilight room lighting
The Philips AmbiLux takes this concept further by using nine pico-projectors on the back of the TV 
% instead
to project an enlarged version of the image~\cite{AmbiLux}. 
Instead of using multiple projectors,
ExtVision~\cite{kimura2018extvision} displays the peripheral context-images using
a single projector mounted on a shelf 6 meters opposite the
TV and 2 m above the ground.
% The context images are generated by a DNN and then cropped
% out its ``inside'' area of   
% The context-images are
% generated and projected onto the peripheral area 
% around the TV by our system.
% They project further than LEDs and, because they aren’t simple lights, can actually reflect the action and motion you see on-screen – the whole image appears to spread across the wall.
% In a follow-up project, Philips created 
% AmibLuxTV, which projects an enlarged image of the television on the wall by a projector attached to the back of the television. 
% The Ambilight system 
Those systems 
mimic 
a larger screen by extending the visual content horizontally and vertically, but limit the experience to the same plane as the main viewing display~\cite{novy2013computational}.
% and restricts it to the low resolution of a single, averaged color per screen edge
Of course, there is a significant boundary discontinuity between the screen and the periphery.

\textit{Head Mounted Displays.}
Although Head-Mounted Displays (HMDs) provide effective immersive experiences for virtual reality,
the FoVs of most contemporary systems are still relatively small 
% (e.g. the Gear VR has roughly 95 degrees FOV).
% compared to the human eye,
and do not fill a user's peripheral field.
% Humans naturally have a horizontal FOV (HFOV) of slightly over 210°. 
% which cannot fully cover a user's peripheral vision.
By adding sparse peripheral displays (SPDs),
% and implemented LED arrays in an HMD. 
 SparseLightVR~\cite{xiao2016augmenting} and Ambiculus~\cite{lubos2016ambiculus}  
can enlarge the FoV to cover approximately 170 horizontal degrees, while SparseLightVR2 improves the HMD's FOV to 180 horizontal degrees~\cite{hashemian2018investigating}.
% Arguably, the most immersive type of display currently available is the HMD. 
% These displays entirely occlude the real world.
% Head-tracking is used to allow the viewer to look around inside the
% space. For real-time rendered graphics, many of these devices allow movement with six degrees of freedom. As most CVR content
% is currently captured, monoscopic, panoramic video, only the three
% degrees of freedom associated with orientation are usually available.
% Regarding the content image generation, 
The DNN-based approach of ExtVision~\cite{kimura2018extvision} 
was adapted for peripheral context generation in 
\cite{kimura2018using}. % HMD contents 
% used deep neural network (DNN) to generate images for peripheral vision and wide FoV customization.
% an effective method for viewing plane videos by an HMD,

% For our implementation, the HMD has 56 RGB
% LEDs (WS2812B) that are individually accessible. The LEDs were
% covered with a thin layer of plastic (ABS, 2 mm thick) produced by
% a 3D printer.

% \textit{Augment Projection Systems.}
\textit{CAVE-like systems.}
% Helmet-mounted displays eventually gave way to less alienating display technologies, such as the
% recursively named C.A.V.E (CAVE automatic virtual environment) system, which projected a synthetic environment on rear projection flats and motion-tracked the user to derive and update
% his or her position in the simulated space [Cruz-Neira].
The system called CAVE (cave automatic virtual environment) 
refers to an immersive virtual reality environment where projectors are directed between three and six walls of a room-sized cube~\cite{cruz1992cave}. 
As compared with affordable and portable HMDs, CAVE-like systems are expensive and require a dedicated, non-portable space. 
% Fortunately, 
% recent years
% have seen a lot of 
% , with developments in projection mapping and Augemented Reality (AR), 
A number of these 
systems have been developed to approximate CAVE-like systems in the home, 
such as 
Infinity-by-nine ~\cite{MITInfinity},
Surround Video~\cite{mills2011surround},
the Microsoft Illumiroom~\cite{jones2013illumiroom}
and RoomAlive projects~\cite{jones2014roomalive}, and Razer’s Project Ariana~\cite{Ariana}.
% provides similar user experience~\cite{philpot2017user}
% Razer. 2017. Project Ariana. (Jan 2017). Retrieved Janurary 9, 2017 from http://www.razerzone.com/project-ariana

% \textbf{Deep generation methods}
% \subsubsection{DNN-based Methods}

% \subsection{Image Completion}
% \subsection{Context Completion Network}
% \subsection{Foveated Framework}
% \section{Two-stage Foveated Framework}

\begin{figure*}[htb] % 18cm for PAMI
\centerline{\includegraphics[width=17.6cm]{framework3.jpg}}
%  \vspace{2.0cm}
\caption{System pipeline of our panoramic image generator. $\oplus$ denotes the image fusion operation.}
% dot lines are only involved in testing phase.
% add generation and fusion part
\label{fig:framework}
\end{figure*}

\begin{figure}[b] % th
\centerline{\includegraphics[height=2.5cm]{cvpr16contextEncoders.jpg}
\includegraphics[height=2.5cm]{cvpr18generativeInpainting.jpg}}
%  \vspace{2.0cm}
\caption{Results using existing inpainting networks. Left: Context Encoder~\cite{pathak2016context}; 
Right: Generative Inpainting~\cite{yu2018generative}.}
\label{fig:inpaint}
\end{figure} 



\subsection{Image Completion}
% To fill in the missing information, we can borrow image completion techniques.
Although the terms ``image inpainting'' and ``image completion'' are often used interchangeably as well as in isolation,
we will use ``image completion'' to mean the union of the concepts of image inpainting and image outpainting. %throughout. % this paper.



% \subsubsection{Traditional Methods}
\textit{Image Outpainting.}
% If the context-image already exists, such as in games, PC work, and movies filmed with dedicated context-capturing
% equipment, we do not need to create it [3, 10]. 
% However, in the case of existing legacy content or content shot without dedicated equipment, it is necessary to estimate and generate
% context-images only from video data. 
Image outpainting has received much less attention~\cite{sabini2018painting} than has image inpainting.
Most existing FoV expansion methods are not suitable for this task, since they require additional images of the same environment, % ~\cite{wang2014biggerpicture,zhang2013framebreak,xia2016novel,shan2014uncrop,sampetoding2018automatic}.
\eg a guide image~\cite{zhang2013framebreak}, two supporting images~\cite{xia2016novel}, or an online/offline image library~\cite{shan2014uncrop, sampetoding2018automatic,wang2014biggerpicture}.
% Mark Sabini and Gili Rusak pro
Although generating context images from the image to be extended using patch/block-matching~\cite{avraham2011ultrawide,turban2017extrafoveal,aides2011multiscale}
is a straight-forward, albeit very different approach, we 
% hope to enhance the process and outcomes by applying DNNs. %for potentially better results.
advance this process and obtain improved outcomes by applying DNNs
trained on substantial amounts of images and context data.
% They state, "wide extrapolations such as those described in the experiments section may take up to several minutes per frame."
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BBC's Surround Video system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \subsubsection{DNN-based Methods}
% \begin{mdframed}[hidealllines=true,backgroundcolor=pink!20]


\csection{pink}{
\textit{Image Inpainting.}
To fill in small or narrow holes in the image to be viewed, propagating neighborhood appearances based on techniques like the isophote direction field is a simple and effective method~\cite{ashikhmin2001synthesizing,ballester2000filling}.
However, these techniques often result in images with significant visual artifacts on large holes.
Alternatively, patch-based methods predict missing regions by searching for 
similar and/or relevant patches from uncorrupted regions of
the image~\cite{barnes2009patchmatch}.
However, a major drawback of these methods %PatchMatch 
lies in the fact that they search for relevant patches based on low-level features over the entire image, without using any context or other high-level information to guide the search. 
% These methods work reasonably well for pure background inpainting tasks where holes are only surrounded by background textures, but could easily fail if holes overlap with an object or are close to an object.
Recent years have seen 
% significant efforts applied to the development of 
% has witnessed 
rapid progress in the field of deep image inpainting
~\cite{iizuka2017globally,liu2018image,yu2018free,yu2018generative,bertalmio2003simultaneous}.
% Can we apply existing inpainting network directly?
% First, I tried existing inpainting methods on this task. 
However, the classical Context Encoder trained on the outpainting task tends to 
produce blurry results, as shown in Fig.~\ref{fig:inpaint}, 
Moreover, while the state-of-the-art Generative Inpainting method~\cite{yu2018generative} can generate clearer images by ``copying'' information based on contextual attention, it often produces unrealistic results when copying foreground information to the background.
Most inpainting networks are not suitable for the outpainting task, since they assume that the missing contents may be drawn from, or are in some way similar to, parts of the original image.
 % small foreground regions. 
Techniques based on such assumptions, \eg contextual attention,
may lead to better inpainting results but worse outpainting outcomes.
%
Finally, techniques that target more challenging inpainting sceneries, such as highly
irregular holes~\cite{liu2018image}, further editing~\cite{yu2018free},
or that seek more visually pleasing inpainting results~\cite{yang2017high,Yan_2018_ECCV,Xiong_2019_CVPR}, 
are not necessary in the outpainting setting.

% We propose a multi-scale neural patch
% synthesis approach based on joint optimization of image
% content and texture constraints, which not only preserves
% contextual structures but also produces high-frequency
% details by matching and adapting patches with the most
% similar mid-layer feature correlations of a deep classification network.
% ~\cite{yang2017high}

% stateof-the-art models, such as PartialConv~\cite{liu2018image} and GatedConv~\cite{yu2018free}. 

% context encoder, the missing parts are predicted by propagating the surrounding convolutional features through a fully connected layer, which intends to produce semantically plausible but blurry result. 

% we introduce a special shift-connection layer to the U-Net architecture, namely Shift-Net, for filling in missing regions of any shape with sharp structures and fine-detailed textures
% Shift-Net
% Deep Feature Rearrangement
% Not needed~\cite{Yan_2018_ECCV}
% Foreground-Aware Image Inpainting~\cite{Xiong_2019_CVPR}


}


\section{System Recommendations}
% \section{Central and Peripheral Vision}
% \subsection{Peripheral Vision Characteristics}

To be able to extend the image content most appropriately and efficiently,
% we need to understand the related human vision capacities and characteristics. 
we make two system recommendations based on 
% related human vision capacities and characteristics.
measurements of visual capacity.
% Since this work only involves images, we don't 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our vision consists of a high resolution fovea in the centre, surrounded by a much more blurry periphery, which has evolved to be good at detecting motion but far worse at fine detail and colour.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The optimal resolution? 512x512 is enough?
%  VR resultion paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% we first make assumptions about the input FoV based on the property of human central vision and then find the output resolution requirements 
% based on human peripheral vision property.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \subsection{FoV and visual experiences.} 
\subsection{Input FoV Recommendation} 
\label{sec:requirement_input_fov} 
% As our target FoV is 180\degree, 
% What's the source Fov?
% To map a single-view image to that of a 180\degree~FoV, 
% First we need to make assumptions about the FoV of source image based on related visual experience studies. 
% Since DNN is efficient at constructing very plausible images, it is compatible with this property of human eyesight.
% The fovea only covers a FoV of $1.5 \degree$ with high visual acuity while 
% the HVS can no longer resolve gratings narrower than 7.5 arc-minutes per pixel by $20 \degree$ of eccentricity
Given an image of a fixed resolution, 
an optimal FoV can be found by finding a best trade-off between image quality and user involvement.
As the gaze of a viewer approaches the image center, s/he will feel more involved as the FoV is increased. However, 
picture flaws arising from a limited resolution become more obvious
as the perceived screen size increases.
% \mydeleted{2}{This mainly involves human visual acuity in the central vision. }
We assume that the input FoV of a single-view-to-panoramic image generation system should be around 50 degrees,
which is the optimal FoV based on 1994 guidelines offered by the Society of Motion Picture and Television Engineers (SMPTE)~\cite{allen1999screen}.
% centeral vision, one pixel wide
% Apparently, we cannot just strech the image to cover a 180 FOV
% Too large a picture leads to excessive grain visibility,
% picture jump and weave visibility, and soft focus.
% the optimal distance from the screen for a good viewing experience based on the viewer’s visual acuity
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Based on the guidelines created in 1994 by the Society of Motion Picture and Television Engineer (SMPTE)~\cite{allen1999screen},
% % the screen delimit a minimum horizontal angle of 30 degree for viewers in the back of the room and 
% the optimal FoV is approximately 50 degree, which corresponds to a viewing distance of 3.45 Picture Heights with the contemporary picture proportions being 1.85:1 for the movie theater~\cite{turban2017extrafoveal}. 
% Intuitively, we assume the input FoV of a single-view-to-panoramic generation system should be around 50 degree. ~\cite{albert2017latency,watson2014formula}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% the optimal FoV is approximately 50 degree, which corresponds to a viewing distance of 3.45 Picture Heights with the contemporary picture proportions being 1.85:1 for the movie theater~\cite{turban2017extrafoveal}. 

% 
% This calculation then leads to a given FoV occupied by the projected image, depending on the screen size, i.e., from 36 degree at the back of a movie theater to 90 degree in the front.
% This corresponds to a distance of 3.45 Picture Heights, using the contemporary picture proportions of 1.85:1 for the movie theater
% Keep this in mind since we will use it when designing our framework.

% \subsection{Spatial frequency sensitivity.} 


\begin{figure}[b]
\centerline{
\includegraphics[width=4cm]{resolution1.png}
\includegraphics[width=4cm]{resolution2.png}} 
%  \vspace{2.0cm}
\caption{Left: the relative resolution. Right: the required resolution (in blue) and the system resolution (in red).}
\label{fig:2resolution}
\end{figure}


\subsection{Output Resolution Recommendation} 
% \textbf{Image resolution and visual experiences.} 
Although the human fovea only occupies 1\% of the retina, this narrow region is very densely populated with photoreceptors, allowing for high-resolution vision in the vicinity of the point of gaze~\cite{kimura2018extvision}. 
By contrast, peripheral vision is much coarser since the density of the photoreceptor decreases rapidly away from the fovea. 
To model the drop-off of resolution in peripheral vision,
we employ the relative spatial frequency function $r: \Theta \rightarrow [0, 1]$ defined in 
\cite{jiang2015salicon}:
\begin{equation}
	r(\theta) = \frac{\beta}{\,\,\,\beta + \theta\,\,\,} ,
\end{equation}
where $\theta$ is visual angle, $\Theta$ is the set of viewing angles with respect to the retinal eccentricity, and $\beta = 2.5\degree$ is the angle corresponding to the visual angle at which
the image becomes only half the resolution of that of the center of gaze ($\theta=0\degree$).
% [0, 1] represents the set of relative spatial frequency. 
% Therefore, the contex image require less resolution 
% contrast sensitivity to higher spatial frequencies drops off as a
% function of retinal eccentricity (e.g., [22, 25]).
This function approximates a normal adult's vision with
the exclusion of the blind spot. 
A higher $r(\theta)$ indicates higher resolution at visual eccentricity $\theta$. 

% Now let's find the recommended resolution for a single-view-to-panoramic system.  
Assume that the viewer's fixation always falls on the original source image, which implies a maximum visual angle of $\theta_1$. The resolution of the input image is assumed to have an uniform, fixed value $R_1$ over the range of visual angles $[0, \theta_1]$. To ensure that the generated peripheral images provide a similar level of visual experience, the resolution at visual angle $\theta_2$ should be at least
\begin{equation}
	R_2 = \frac{r(\theta_2-\theta_1)}{r(\theta_1-\theta_1)} R_1 = \frac{\beta}{\beta+\theta_2-\theta_1} R_1.
\end{equation}
We plot the recommended relative resolution in Fig.~\ref{fig:2resolution} for an optimal visual angle 25\degree(half of the optimal FoV). 
% In such cases, the 


% \subsection{Foveated Framework}




\section{System Implementation}
% SYSTEM RECOMMENDATIONS
\label{sec:ourApproach}


As shown in Fig.~\ref{fig:framework}, our approach 
% is based on a two-stage foveated framework and 
comprises two main processing modules: generation and fusion. 
First, %a resized version of 
the input is fed into the generation module, generating two separate outputs that correspond to a 90\degree~FoV and a 180\degree~FoV, respectively.
Then, the fusion module fuses the input image with the two outputs to create a panoramic image, which includes the blending process.
% Finally, the fusion result is mapped to the half sphere for viewing.
Finally, the fusion result is mapped to the sphere for viewing.
We use the commonly used equirectangular projection as the format for storing panoramic image data.





\subsection{Two-stage Foveated Framework}
% \subsection{Divide and Conquer}
% Instead of  , 
We divide the foveated image generation problem into two stages, as depicted in Fig.~\ref{fig:2stage}(c).
In the first stage, we extend the image to twice its original size, %just like ExtVision~\cite{kimura2018extvision}.
thereby expanding the FoV to 90\degree.
In the second stage, we further expand the FoV from 90\degree to 180\degree.
% As the spatial frequency sensitivity of the HVS drops off 
% dramatically as the stimulus is moved 
% away from the fovea and into the periphery,
% We can use successively decreasing resolutions for the three regions.
% we can use two resolution levels as aforementioned.
We use two stages rather than one based on two observations:

\begin{figure}[t]
\centerline{\includegraphics[width=7.6cm]{2stage2.jpg}}
\vspace{-2mm}
% \centerline{
% \includegraphics[width=7.2cm]{central-peripheral.jpg}}
\caption{Two-stage foveated framework. 
\textit{G-I} is the central-to-near-peripheral generator and 
\textit{G-II} is the near-to-mid-peripheral generator.
}
\label{fig:2stage}
\end{figure}
% goes through


\begin{itemize}[noitemsep,leftmargin=*]
	% \itemsep0em
	\item[--] %To meet the resolution requirements,
	The system requires at least two resolution levels, as shown in Fig.~\ref{fig:2resolution}. This means that if only a low-resolution context image is generated, the viewer will notice the sudden resolution fall-off at the boundary. To alleviate this problem, we can sacrifice a small portion of the original image to form a transition region. Alternatively, if we first outpaint the image to a larger size, then the outpainted region can include the transition region, without reducing the original image.
	% visual experience falloffs in areas 
	% : A transition region with linear density falloff between the fovea and far periphery,
	% \item[--] 
	As shown in Fig.~\ref{fig:2stage}(b)(c), the final image consists of three regions that roughly correspond, respectively, to the center (0$\sim$50\degree~FoV), the near periphery (50\degree$\sim$110\degree~FoV), and the mid periphery (110\degree$\sim$170\degree~FoV). 
	% We can add special design for different regions according to human vision capacities and characteristics. 
	% % In the following subsections, 
	% We will show the benefits of this ``divide-and-conquer" strategy in Sect.~\ref{sec:divide-and-conquer}. 
	\item[--] 
	% Here 90\degree is not a random choice. 
	Although VR devices provide 360\degree of freedom for viewing, a user can only view 90\degree~at a time on most contemporary devices. On images generated using our framework, a user only sees the generated 90\degree~image when fixating at image center.
\end{itemize}
% Therefore, we present a two-stage foveated framework. We will introduce more advantages about the two-stage setting in the following subsections.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% You can only see 90 degrees at a time.
% While 360 video features a complete panoramic 360-degree horizontal view and a 180-degree vertical view, it’s important to understand that on most Head Mounted Displays (HMD) a user can only see about 90 degrees at a time. 
% Viewing the entire sphere of the video involves the user turning and tilting their head and body.At any given moment, a viewer can only see about one-quarter of an immersive video– the slice of the image directly in front of them.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Before describing the implementation details, 
we show that the two-stage framework meets our system requirements.
In the first stage, we map the normal FoV to a 90-degree FoV.
\begin{figure}[b]
\centerline{\includegraphics[width=7cm]{fov_setup.jpg}}
%  \vspace{2.0cm}
\caption{Calculation of the input FoV of our system. $O$ is the image center and $P$ is the location of the viewer. }
% \caption{FoV setup.}
\label{fig:fov}
\end{figure}
As shown in Fig.~\ref{fig:fov}, 
$ABCD$ is the original image, and we extend the FoV by 
% simply 
extending the image both horizontally and vertically, yielding a 4-fold larger image $A'B'C'D'$. 
Given the target FoV $\alpha'$ of 90\degree, we have 
\begin{equation}
	\frac{EF}{E'F'} = \frac{OE}{OE'} =  \frac{OP \times \tan (\alpha/2)}{OP \times \tan (\alpha'/2)} = \frac{ \tan (\alpha/2)}{\tan (\alpha'/2)}.
\end{equation}
The input FoV is around 50\degree, which meets the requirement stated in Sect.~\ref{sec:requirement_input_fov}:
\begin{equation}
	% \alpha = 2 \arctan ( \frac{EF}{E'F'} \tan \frac{\alpha'}{2} ) = \frac{1}{2} \arctan(2 \tan \frac{90\degree}{2} ) \approx 53.13\degree 
	\alpha = 2 \arctan ( \frac{EF}{E'F'} \tan \frac{\alpha'}{2} ) = 2 \arctan (\frac{1}{2} \tan \frac{90\degree}{2} ) \approx 53.13\degree 
\end{equation}
Regarding the output resolution, the near periphery region has the same resolution as the input, whereas the mid periphery has a lower resolution:
\begin{equation}% (2.5)/(2.5+90/2-53.13/2)
	% R_1 \ge \frac{\beta+\theta_0}{\beta+\theta_1} R_0 = \frac{2.5\degree/2}{2.5\degree+90\degree/2} R_0 \approx 0.12 R_0.
	R_2 \ge  %\frac{\beta}{\beta+\theta_1-\theta_0} R_0 = 
	\frac{2.5\degree}{2.5\degree+90\degree/2-53.13\degree/2} R_1 \approx 0.12 R_1.
\end{equation}
Following the second stage, the output resolution is about half that of the input, which greatly exceeds our requirements. 
% For implementation, one 
Therefore, we can resize the image output from stage 2 by a factor of 4 to reduce computation. 

% accurate but 
% a large amount of inaccurate data
% Foveated rendering techniques use similar 
% Recusively painting vs two-stage painting
% one stage painting

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
% \centerline{\includegraphics[width=7cm]{extvision_method1.png}}
% \center(a) Method 1: Category-limited method\\
% \centerline{\includegraphics[width=7cm]{extvision_method2.png}}
% \center (b) Method 2: Recursive method
% \caption{Results of ExtVision.}
% \label{fig:inpaint}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% figure- Category-limited method and Recursive method

\input{ablation_studies}

\subsection{Generation Module}

% For each sub task, we train a network to 
As mentioned earlier, there are two stages in the generation module:
near-periphery generation and mid-periphery generation.
Both stages can be formulated as an outpainting problem, while the latter one also involves a geometric transformation.
% We train two generators for those two stages.
% The first generator takes in the input image and expand it twice horizontally and vertically.
% % outputing an image with twice width of the input.
% The second generator map a 90\degree perspective image to a 180\degree panoramic image.

% Therefore, we need a database, network and a training 


\subsubsection{Network Architecture}
% With enough training data, the next problem is a suitable network architecture.
% In this subsection, we first give a brief remark on whether existing deep image completion networks is suitable for this task
 % Image completion and inpainting are closely related technologies used to fill in missing or corrupted parts of images. There are many ways to do content-aware fill, image completion, and inpainting.
% Take Contextual Attention proposed in \cite{yu2018generative} as an example, the basic idea is to borrow or copy feature information from known background patches. However, no background patches available in our cases.
% Therefore, we didn't employ inpainting techniques and
% Extrapolating, Field-of-View Expansion, Uncrop, Extrafoveal Video Extension
% Fortunately, achieve  based on .
% As discussed in Sect.\ref{sec:relatedWork}, existing inpainting network can not directly applied to this task.
We employed pix2pix~\cite{pix2pix2017}, which has been shown to deliver visually appealing results on the image outpainting problem~\cite{kimura2018extvision}, as our network architecture.
% Pix2pix learns image-to-image transformation by a conditional Generative adversarial network(cGAN) architecture.
Pix2pix has also been used to learn various image-to-image transformation such as ``black and white image to color image,'' ``edge map to natural image,'' and ``aerial photograph to illustrated map,'' and so on.
We independently trained two networks, using the pix2pix architecture to learn narrow-to-90\degree peripheral image generation 
and 90\degree-to-180\degree peripheral image generation.
% Regarding the training pipeline, 
% we trained the two networks independently. 
% \note{I will confirm this by doing more experiments}
% \mydeleted{2}
% {We also tried jointly training as a refinement step, 
% but we didn't adopt it since it brings no obvious improvement.}
% \ctext[RGB]{255,165,0}
\csection{orange!40}{We chose the U-Net~\cite{ronneberger2015u} as the generator network in pix2pix, since it gives better results as compared with ResNet~\cite{he2016deep} alternatives, in terms of NRMSE and PSNR between generated images and ground truth images (\cf Table~\ref{tbl:resnet_vs_unet}).}




% We address the problem of extending the field of view of a photo— an operation we call uncrop. Given a reference photograph to be uncropped, our approach selects, reprojects, and composites a subset of Internet imagery taken near the reference into a larger image around the reference using the underlying scene geometry.
% significantly extrapolate the field of view of a photograph
% by learning from a roughly aligned, wide-angle guide
% image of the same scene category.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In recent years, image completion technologies using Deep Neural Networks, especially convolutional neural networks (CNN), have experienced significant progress [7, 13]. Image completion means to fill a “hole” and to attempt to restore lost image data. The model proposed by Iizuka, et al. [7] succeeded in complementing a natural image such that it could not be recognized as “filled” at a glance. We assume that the peripheral imagery can be filled in approximately the same way by applying a mask to the peripheral portion and treating it as a “hole.”
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Viewing full spherical is a natural medium to be explored in VR.

% In this paper, we describe how images are displayed as context-images in peripheral areas to enhance visual experiences. 
% Illumiroom [10] projects context-images or visual effects around the TV screen and enhances the traditional gaming experience. 
% ScreenX [20] and BarcoEscape [21] provide sub-screens to display video on both sides of the main screen, providing a more immersive movie experience.

\forjrnl{
\subsubsection{Loss Function} % and Training Pipeline

To produce a visually pleasing outputs, it is necessary to define a suitable loss function.
% Can be other realistic result similar to 
% How can we define realistic?
% The generator 
We use the same loss function as was adopted in Pix2pix when training two networks.
Pix2pix is a conditional Generative adversarial network(cGAN),
optimizing a generator $G$ by competing with %fooling 
a discriminator $D$ in a min-max game:
% adversarial learning techniques:
% generating both realistic and controlled outputs by 
% the optimal Generator $G$ is found by
\begin{equation}
	G^* = \text{arg} \min_G \max_D \mathcal{L}_{cGAN}(G, D) + \lambda \mathcal{L}_{L1} (G),
\end{equation}
where $G$ tries to minimize the loss function against $D$, which tries to maximize it. 
The loss function relatively weights the GAN loss and the L1 loss using the control parameter $\lambda$.
% Denote the generated result as $y^*$ and the ground truth $y$,
The GAN loss describes the accuracy of $D$ in differentiating fake samples $y^*$ generated by $G$ and real samples $y$:
% is defined as
\begin{equation}
	\mathcal{L}_{cGAN}(G, D) = \EX_y[\log D(y)] + \EX_{y^*}[\log (1-D(y^*))],
\end{equation}
while the L1 loss constrains the output to fall close to the ground truth:
\begin{equation}
	\mathcal{L}_{L1} (G) = \EX_{y,y^*}[||y-y^*||_1],
\end{equation} 
% 255,165,0
where $||.||_1$ is the $\ell_1$ norm.}\csection{orange!40}{We also tried 
% other GAN loss functions,
the L2 loss in LSGAN~{\cite{mao2017least}}, but it produces blurry results due to averaging of the possibilities~{\cite{larsen2015autoencoding}}.
Using WGAN loss~{\cite{arjovsky2017wasserstein}} gives sharp results, but it tends to produce artifacts.
Therefore, we use the vanilla GAN loss in our method.}%


\subsection{Fusion Module}

To obtain the final panoramic image,
first fuse the input with the generated near periphery image, 
then fuse the result with the generated mid-periphery image.
Before fusing, the images are padded with zeros so they can be aligned on matching domains. 
We used Poisson blending technique
% the modified Poisson blending technique~\cite{afifi2015mpb}
~\cite{perez2003poisson} to obtain better fusion results, as shown in Fig.~\ref{fig:blend}.


\begin{figure}
\centering

% \begin{subfigure}[b]{.4\textwidth}
% \centering
% \includegraphics[width=.4\textwidth]{example-image}\quad
% \includegraphics[width=.4\textwidth]{example-image}

% \caption{}
% \end{subfigure}\quad
% \begin{subfigure}[b]{.4\textwidth}
% \centering
% \includegraphics[width=.4\textwidth]{example-image}\quad
% \includegraphics[width=.4\textwidth]{example-image}

% \caption{}
% \end{subfigure}
% \centerline{ % 3.8 --> 3.6
% \includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_context_noblend.jpg}
% \includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_pano_noblend.jpg}
% }
% \centerline{
% \includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_context_blend.jpg}
% \includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_pano_blend.jpg}
% }
\begin{picture}(103,103)
\put(0,0){\includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_context_noblend.jpg}}
\put(10,90){without blending}
\end{picture}
\begin{picture}(103,103)
\put(0,0){\includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_pano_noblend.jpg}}
\put(10,90){without blending}
\end{picture}
\\
\begin{picture}(103,103)
\put(0,0){\includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_context_blend.jpg}}
\put(10,90){with blending}
\end{picture}
\begin{picture}(103,103)
\put(0,0){\includegraphics[height=3.6cm]{pano_afdshrfpqnhibr_back_fake_pano_blend.jpg}}
\put(10,90){with blending}
\end{picture}

\caption{Left: Near periphery fusion with and without blending.
Right: Mid periphery fusion with and without blending.}
\label{fig:blend}
\end{figure}



% \subsubsection{Continuity Vs. }

\subsubsection{Divide and Conquer}
\label{sec:divide-and-conquer}
% We fill each regions using different strategies. 
% advantage of two-stage
% Regardless of the proposed resolution requirement, 
\ctext[RGB]{255,255,204}{While training a single generator to predict the 180\degree~image from the input image would seem to be a straightforward solution, 
we have found that training two generators to conduct image extrapolation, and 90\degree to 180\degree~predication, respectively yields better results.
% respectively would be a better ....
% By dividing it into two sub problems,
% However, it has two problems: 1. the region corresponding to near periphery cannot meet the resolution requirement; 2. the dis
% two sub tasks,
% However, we found it would give better fusion results if we divided 
In our framework, the final
image consists of three parts: the original input image, the generated near peripheral image, and the generated mid peripheral image respectively.
% we fuse the input image with two generated images corresponding to the near and mid periphery respectively. 
This divide and conquer strategy breaks the challenging image generation problem into two parts having different requirements.
% and handled by two generators. 
% stages/parts:  
The near peripheral image requires not only a higher resolution, but also less distortion as compared with the mid peripheral image.
}
When fusing the generated peripheral context images with the original images, we noticed that 
the outputs of the mid periphery generation network 
yielded relatively poorer continuity with their inputs as
compared with those produced by the near periphery generation network.
This is probably because the mid-periphery generator conducts both image outpainting 
as well as geometric transformation.
Continuity is much more difficult to preserve 
while also accounting for geometric inconsistencies between the inputs and outputs.
Fortunately, the viewers are unlikely to perceive this discontinuity 
when fixating at the image center, 
since 90 degrees of FoV are covered by the generated near-periphery image.
%
% We divide the challenging single-view to panoramic problem 
% Sine the context discontinuity in transition region is more sp than the 
% Consistency is more important
% Presence is more important
The divide and conquer strategy is more efficient than only using outpainting or direct panoramic mapping.
If we were to use this network to map the input to 180\degree~directly,
the discontinuity would become more obvious and could adversely affect the user experience.
It would also be more storage-intensive and time-consuming 
to generate the 180\degree~image by recursively applying the outpainting network.
% Combining those two networks 
% Since both outpainting and pano painting has their strength and 
% limitation, we combine them together.

%%%%%%%%%%%%%%%%%%%%%%% TODO, this point is also important !!!!!!!!!!!!
% Why not just do outpainting recusively and then map the result to sphere?
% The problem of recursive outpainting.
% and also, the recursively outpainting has some issue. show pictures!!!!! [DO it in journal version]
% Another reason why directly panoramic mapping is not recommended
% is that 
% the near periphery region has higer requirement, and can be learn by using the input video. thus provide a better 
% the requirement 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\input{fig_halo}
\input{fig_single_cat_results.tex}

\subsubsection{Preprocessing and Postprocessing}
\label{sec:pre-and-post}
% In this section, we discuss the additional modification to improve the fusion results.
\ctext[RGB]{255,255,204}{In ExtVision, 
% of the extrapolated image
the input and the output of the generator are aligned by zero-padding the input.}
As shown in Fig.~\ref{fig:halo}, this may introduce halo artifacts at the image boundaries, since the generator tends to directly copy from the input because of 
the skip connection of the pix2pix architecture.
To avoid direct copying by breaking the alignment,
we resize the input instead of zero-padding, leading to better fusion results (see Sect.~\ref{sec:results}).
% before feeding into the generator 





% regions to be filled 
% Related Definitions
% \section{single-view-to-panoramic-image-generation methods}

% For rectangular image, we will first resize 
% We first resize the image into square size, then put it 
% into a 53.13\degree lk
% 3-resolution Foveated extrapolation
% 3-resolution is not accurate, better use 3-region

% Video extrapolation is the task of extending a video beyond
% its original field of view. Extrapolating video in a manner
% that is consistent with the original video and visually
% pleasing is difcult. In this work we aim at very wide video
% extrapolation which increases the complexity of the task.
% \cite{aides2011multiscale} 

%% Foveated video extrapolation
% Foveated video extrapolation reduces the effective
% number of pixels that need to be extrapolated, making
% the extrapolation less time consuming and less prone to
% artifacts. The coarse to ne approach better preserves the
% structure of the scene while preserving ner details near the
% domain of the input video. The combined method gains improvement
% both visually and in processing time.

% VR system follows a 
% don't perform eye tracking

%% Foveated rendering
% Foveated rendering is a performance optimization based on the well-known degradation of peripheral visual acuity. It reduces
% computational costs by showing a high-quality image in the user’s central (foveal) vision and a lower quality image in the
% periphery. Foveated rendering is a promising optimization for Virtual Reality (VR) graphics, and generally requires accurate
% and low-latency eye tracking to ensure correctness even when a user makes large, fast eye movements such as saccades.
% However, due to the phenomenon of saccadic omission, it is possible that these requirements may be relaxed.
% https://research.nvidia.com/sites/default/files/pubs/2017-09_Latency-Requirements-for/a25-albert.pdf

% At the time of this
% writing, the best VR displays have a resolution of 1080 × 1200 pixels per eye
% The Field of View (FoV) of current displays is limited to 100◦ horizontally,
% which is only half of the binocular horizontal FoV of the human visual system

% Many VR
% applications also require stereo depth information, doubling rendering costs, and perceptual research in flicker

% Divide and conquar
% Like VR foveted rendering systems~\cite{albert2017latency}, 
% we divide the visual field in to three regions based on retinal eccentricity:

% % foveation density mappings
% \setlist{nolistsep}
% \begin{itemize}[noitemsep]
% 	% \itemsep0em
% 	\item[--] Fovea: A uniformly high-density region from the gaze center to two-thirds of the corresponding farperipheral eccentricity, i.e., 3.33◦, 6.67◦, and 13.33◦, respectively.
% 	\item[--] Far Periphery: A uniformly low-density region beyond a fixed eccentricity of either 5◦, 10◦, or 20◦.
% 	\item[--] Transition Region: A transition region with linear density falloff between the fovea and far periphery,
% one-third of the far-peripheral eccentricity in size.
% \end{itemize}

% Figure 3 shows our three foveation density mappings
%  remove the cnnection my leads to blurry outputs

%  read the pix2pix paper and then write here
% Augmumentation?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% image that are not square
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[b]
% \centerline{\includegraphics[height=8cm]{post-processing.jpg}}
% %  \vspace{2.0cm}
% \caption{Post-processing.}
% \label{fig:post-processing}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% image that are not square END
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Other details}
% \subsubsection{360-degree image generation}
Since most VR devices only provide 90\degree of viewing at any moment, a 180\degree~output is adequate provided that the viewer's fixation lies within the region of the input image.
However, outputs having a FoV larger than 180\degree~may be required %for a better visual experience 
in some peripheral presentation systems,
since a viewer's effective FoV can reach 270 degrees with rotation of the eyes and even further with head rotation~\cite{turban2017extrafoveal}.
% Although an eye’s theoretical forward-facing horizontal FoV is around 180 dgree, 
% However, peripheral presentation systems can provide 360\degree at a time.
% and up to 270 degree with eyeball rotation (head rotation excluded).
In such cases, we can extend the generated 180-degree images to 360 degrees by simply applying a mirror reflected copy operation.

% For images that are not square, 
% Assume an 128$\times$128 input, for image with arbitrary size, we first resize it into 256$\times$256

% \lipsum[2]


% Comments on Applying this techniques to video
% increased sensitivity to flicker, we need to avearage frames.
% as shown in Fig.~\ref{fig:180to360}.

% As for stereoscopic images/videos, can share 

%%%%%%% no space for this figure.... 
% \begin{figure}[htb]
% \centerline{\includegraphics[width=8.5cm]{intro.png}}
% %  \vspace{2.0cm}
% \caption{Extend 180-degree to 360-degree by replication.}
% \label{fig:180to360}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%

% Blur the background, pop out the foreground
% Foveated rendering allows the peripheral image to be degraded in a way that decreases
% computation and is perceptually unobtrusive. 

% This requires gaze tracking, and therefore foveated systems are
% very sensitive to latency



\input{fig_more_results}



\section{Evaluation}
% \section{Experimental Results}
\label{sec:results}
% In this section, we evaluate our method(method name abbr?)%
 % with comparison to the state of the art approaches 
 % and ablation study to fully investigate the proposed method.

% Due to the lack of any meaningful performance metrics,
% which is an interesting problem itself,
%  % for this new task,
% we are only able to provide a number of examples and visual comparisons. 

% \begin{mdframed}[hidealllines=true,backgroundcolor=green!20,leftmargin=-6pt,rightmargin=-6pt]
% 
\csection{green!20}{
We trained two generators on image pairs extracted from SUN360 datasets (\cf Sect.~\ref{sec:database}).
As shown in Fig.~\ref{fig:2stage}(c), 
the first generator produces content for the near periphery (colored in blue) while the second generator produces content for the mid periphery (colored in green).
% When training, 
For the second generator, the input image has a normal field of view while the target image has an 
equirectangular form. Therefore, geometric translation is involved in addition to image generation. 
% }
% \end{mdframed}
}



% \begin{figure*}[tbh]
% \centerline{\includegraphics[height=10cm]{outdoor.png}}
% %  \vspace{2.0cm}
% \caption{More results on diverse scenes. The first row shows the input images while the next row shows the generated outputs using our method. Images are from the test set, i.e. the \texttt{others} category of the SUN360 dataset.}
% \label{fig:res_outdoor}
% \end{figure*}


% \begin{figure*}[bth]
% \centerline{\includegraphics[height=10cm]{indoor.png}}
% %  \vspace{2.0cm}
% \caption{More results on diverse scenes. The first row shows the input images while the next row shows the generated outputs using our method. Images are from the test set, i.e. the \texttt{others} category of the SUN360 dataset.}
% \label{fig:res_indoor}
% \end{figure*}

% \subsection{Ablation Study}
% % \subsection{Ablation Study}
% Very different system.

% Not all methods have stage 1 or stage 2, so just use the final result
% for each stage, we may also report their difference.

% S-PSNR [24]
% Windowed S-PSNR [27]

% Sphere comparison. 





\subsection{Datasets}
\label{sec:database}
% \begin{mdframed}[hidealllines=true,backgroundcolor=red!20,leftmargin=-6pt,rightmargin=-6pt]
\csection{red!20}{
% in this section, we don't mention resize operation, we don't limit the network input now.
% To train a good deep network 
Since most DNN-based methods are data hungry, it is necessary to feed enough data to the networks so that they may learn a sufficiently substantial peripheral representation space.
We used the SUN360 dataset~\cite{xiao2012sun360}, which provides diverse panoramic image resolutions up to $9104\times4552$.
% and their performance is strongly correlated with the amount of available training data.
% For near-peripheral generation, 
% we used the $256\times256$ version of the Places2 dataset~\cite{zhou2017places}. 
% The Places2 training set contains 1,803,460 images, with 5000 to 30,000 images within each category.
% We use category-limited or recursive strategy proposed in ExtVision to get a better result and shorter training time. 				
% As in ExtVision, xxxx, forming an input-output pair.
% We use cropped data as input...
% slice an image patch from a panoramic and map it to a single view(from
% FoV 90 ◦ back to FoV 0 50 ◦ ) as the target of the first module.
% SUN360 dataset provides upto $9104\times4552$ resolution, 
% we use $1024\times512$ vesion
For each panoramic image, we selected four input-output pairs: front, back, left, and right. 
For each direction we generated a pair of images that correspond to an FoV of 90\degree, and an FoV of 180\degree, respectively.
Those two images were resized to $256\times256$ and fed into the mid periphery generator as input and target, respectively.
For the near periphery generator,
the 90\degree~image and its central 1/4 portion were are also resized to $256\times256$ and fed as target and input respectively.
The SUN360 dataset provides 14358 indoor images, 52938 outdoor images, and 274 other images.
We fused the indoor category with the outdoor category, and held out 100 images for validation. 
The overall training set contains $268,784$ input-output pairs. % 4\times(67296-100)=
% \end{mdframed}
}
% Both are resized to $256\times256$ and then feed into the network.
%

% \subsection{Training Parameters}

% The model is optimized via the mini-batch stochastic
% gradient descent (SGD) with backpropagation. We set
% batch size of SGD to 64, momentum parameter to 0.9 and
% weight decay to 10 -4 . We use the method described in [11]
% to initialize the weight of the convolutional filters. The
% weight of the transposed convolutional filter is initialized
% from bilinear interpolation kernel. The initial learning rate is
% set to 0.1 and then decreased by a factor of 10 every 20
% epochs. Due to using a large learning rate during the training
% session, we adopt the gradient clipping [12] to restrain
% gradient explosion. Specifically, the gradients are clipped to
% 0.4. We train our model with PyTorch [14], which is a deep
% learning framework.



\subsection{Sample Results}



% \lipsum[2]
% \subsection{Limitations}

% Fig.~\ref{fig:res_outdoor} shows single-category results. 
% ProGAN (Karras et al., 2018) trains high-resolution GANs in the single-class
% setting by training a single model across a sequence of increasing resolutions.
The results we obtained using the model trained on images in a specific category are shown in Fig.~\ref{fig:res_outdoor}.
Results using the model trained on the entire training set of all categories are given in Fig.~\ref{fig:demo}.
Since GANs trained on a single category can capture a more accurate 
distribution as compared with training on images from multiple categories,
there is an obvious performance gap between the single-category results and the multiple-category results.
% Multi-category Results
% \subsection{Cross-category Results}
When making comparisons, it is important to remember the exemplars shown on the pages here will appear very different when viewed immersively, especially in the periphery.
Nevertheless,
the cross-category results are often less acceptable, although very good results are obtained when the categories are similar.
% Another limitation of the proposed method is that 
% the its generation abilities to unseen data.  % learning-based method
% It means that the networks can not 

Naturally, it is difficult for a network to generalize well from training data to unseen data.
For example, we trained a model only using indoor images, then applied it to the outdoor database.
The model tended to draw a ceiling on the top of the rendered output image, since it is very common in the training set.
For the central-to-near-peripheral generator, we can use the recursive method~\cite{kimura2018extvision} to avoid this problem when the input image is from a video.
Specifically, we crop the video frames to form original image and cropped image pairs as a training set.
However, since all frames have a limited FoV, we could not use this trick for near-to-mid-peripheral generation, which requires a 180\degree~FoV ground truth.
Another limitation is the input resolution.
Currently, our networks cannot produce context images inputs larger than $128\times128$, since they only accept a fixed-size input of 256$\times$256.
% The output resolution may not meet the requirement if the input images are resized.
% We can get an output image that 
This limitation can be addressed by modifying the network architecture, \eg by adopting fully-convolutional neural networks that can accept images of different resolutions.
%
% Therefore, we need to make sure the input image 
% Matching unknown input ....  
% produce bad results.

% [additional experiment analysis will be added here.]
% \\ ... 
% \\ ... 
% \\ ...
% \\ ...
% \\ ...
% \\ ...
% \\ ...
% [additional experiment analysis will be added here.]

% \subsection{Single-category Results}
% \subsection{Multi-category Results}
% \subsection{Cross-category Results}





\input{PSNR_NRMSE}



\subsection{Comparison with Existing Systems}

% \subsection{Applications}
% \subsubsection{Adapted to existing systems}
% \subsubsection{Competing Approaches}

We compared against results obtained by two state-of-the art approaches for image outpainting. Multiscale is PatchMatch-based; while ExtVision is DNN-based.

\textit{Multiscale}~\cite{aides2011multiscale}.
% The Multsicale Ultrawide Foveated Video Extrapolation method proposed by Aides et al. [9] solved a large number of these issues. 
% The key idea of their algorithm, developed from an original work by Avraham and Schechner~\cite{avraham2011ultrawide}, is to use a PatchMatch algorithm in space and time dimensions to extrapolate the video to outside of its borders. 
This is a PatchMatch-based video extrapolation method proposed 
by Aides \etal, as an improved version of their earlier work~\cite{avraham2011ultrawide}. 
Both methods use a foveated framework to imitating the resolution variation of the human fovea.
The resolution of the extrapolated video diminishes
toward the boundaries of the extrapolated region.
% The original work also follows a multi-scale manner,
 % but 
The process
starts at the finest resolution level, 
\ie the innermost domain, 
and proceeds outwards from fine to coarse. 
% We refer to it as an Inside-Out method. 
% The video extrapolated over each inner domain is used as the input video for the extrapolation of the next, coarser and outer, domain. While it successfully showed reduction in artifacts and processing time, the Inside-Out method has several shortcomings.
% This leads to several shortcomings such as
To improve the scene structure and to better preserve texture, Multiscale instead performs a coarse to fine completion.
Although 
the search for an appropriate patch is limited to within a certain area of the original video to reduce computation time,
this approach still requires several minutes to extrapolate one frame, and some artifacts may remain.

% Here, multi-scale means In order to better adapt to human vision, which is less sensitive to detail when farther from the center of the retina, the algorithm was computed at different resolutions. The best results were obtained when the extrapolation was performed from the coarsest resolution to the highest. 
% In choosing the right patch, they also penalize the patches likely to cause distraction, i.e., those that add many edges outside of the video. The patch used is also selected randomly among a small number with a similar reconstruction cost in order to avoid an unnatural repetition of the same patch. To limit computation time, the search for an appropriate patch is limited to a certain area in the original input video, closest to the missing pixels that are being filled, with this area then being extended if necessary. 
% This algorithm has one negative, however: its high complexity, as it takes several minutes to extrapolate one frame and some artifacts still remain in some cases.




\textit{ExtVision}~\cite{kimura2018extvision}.
% Unlike Painting Outside the Box~\cite{sabini2018painting} extends the 
This work described two methods using a DNN to generate
peripheral context-images for videos:
a category-limited method and a recursive method.
The former uses a network trained on the same category, 
while the latter uses a network trained on the original video frames.
Since we are mainly interested in immersive still images, 
% instead of videos in this paper, 
we use the first method as a comparison.
% With our methods, a patch size of 256 × 256 pixels
% allows the most natural reconstruction of images (i.e., the
As compared to time-consuming PatchMatch-based approaches, ExtVision ensures a processing speed suitable for real
time generation (30 fps).
% and faster than conventional methods
The concurrent work by Sabini et al.~\cite{sabini2018painting} also treats image outpainting using deep learning algorithms,
but only extends the images horizontally.
% Besides, the results and feedback from user tests shows that the same effects as the Illumiroom system can be obtained for peripheral projection of existing context-images,
% as well as the type of videos are well-suited ExtVision system.

% \subsubsection{Results}%


Fig.~\ref{fig:comparison} shows exemplar results compared to existing methods. 
% Although  
ExtVision~\cite{kimura2018extvision} causes discontinuities to appear at the connection boundaries, because of the direct copy phenomenon mentioned in Sect.~\ref{sec:pre-and-post}.
Multiscale~\cite{aides2011multiscale} is a video extrapolation method which requires neighboring frames as inputs.
% Based on the proposed two-stage framework, 
Our method achieves a more immersive and visual pleasing result,
without boundary artifacts and without requiring other frames.
% More generation results can be found in Fig.~\ref{fig:demo}.

% \subsubsection{Computation Time}
% the fuse and the geneartion can be done simutanously
% the stage 2 can use the output image of stage 1 in last frame,
% use pipeline 

% The time needed for processing 1200 images was around 30
% – 35 seconds on models created by our methods. In this study,
% we evaluated our method on a PC using an Intel Core i7-
% 5930K CPU with NVIDIA GeForce TITAN X GPU. All
% such the models we generated in this paper could process over 30
% fps, which is common for TV contents or movies. As a

% Although we can’t make exact comparisons because
% experiments were not done in the same environment and the
% Multiscale method’s speed varies according to the settings
% as the number of frames to be searched and the
% resolution
% of the input image, our methods are much faster





\csection{blue!20}{
% \begin{mdframed}[hidealllines=true,backgroundcolor=blue!20,leftmargin=-6pt,rightmargin=-6pt]
\input{human_study}
% \end{mdframed}
}





\section{Conclusions and Future Work}
\label{sec:conlusions}
\label{sec:futureWork}

% In this paper,
We were able to successfully realize a single-view-to-panoramic image generation system using a deep learning approach. 
% we need more proofs!
Regarding this challenging task, two system recommendations, a two-stage foveated framework and a DNN-based approach were proposed.
 % to predict visually appealing results.
While our current approach was created in the context of monoscopic images, the same or similar approaches could be used
to enhance immersive stereoscopic images and videos.
Our proposed method could also be easily applied to video extrapolation in a frame-by-frame manner, mapping a single-view video to a panoramic video.
Since peripheral vision is highly sensitive to flicker~\cite{tyler1987analysis}, a time smoothing filter that averages neighbor frames could be employed 
% as a post-processing step 
to alleviate any flicker problems,
as was done in ExtVision~\cite{kimura2018extvision}.
% \myadded{2}{
% % All in all, if we can generate a panoramic context image from a single-view image, both peripheral presentation systems and VR systems will benefit. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Open Source                    %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% To encourage future work on this new task
% and allow more experimental verification and comparisons, 
% we will make the source code open at Github. 
% Interactive demos, code, and data can be found on our project website~\footnote{The link will be provided after the double-blind review process. Please see Supplementary Information for some additional results.}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  Open Source                    %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% videos, 
% We provide open source interpretation tools to help peer researchers and practitioners better understand their GAN models
%  and data are available at GitHub and gandissect.csail.mit.edu.

% We show that single-view-to-panoramic with deep learning 
% is both feasible and promising.
% This technique can be applied to not only peripheral presentation systems
% but also virtual reality (VR) devices.
% % In contrast to 
% Unlike peripheral presentation systems, 
% VR devices are becoming more and more popular these years.
% By utilizing stitching algorithms that takes multiple video streams together and outputs a 360 degree video,
% VR devices support 360\degree content FoV and provide an a new generation of visual experiences.
% % [wrong !!! only 90 fov one time].
% But when it comes to the creation of such 360 degree videos, it is not only money and time consuming because of special capture devices
% but also challenging or even impossible because of the limitation of shooting sceneries and stitching algorithms.
% % With the proposed method, we can generates VR content from traditional narrow-angle videos,  
% Single-view-to-panoramic techniques have great potential to 
% generate VR contents transformed from the large amount of legacy narrow-angle contents, ready for enhanced viewing on VR displays.
% }
% Although -
% In our study, 
% it was found that our method could generate context-images that were considered consistent with the inside videos while keeping processing speeds that were fast enough for the real-time generation. However, several problems remain. First, in order to realize strict real-time processing, it is necessary to increase the generality of generation. Method 1 requires users to select suitable models for the video. On the other hand, Method 2 needs long learning times for each video. If no one has trained the model and there is no pre-trained model in the world, processing time should include the very long learning time. Therefore, we need to create a generic model that can properly process any image. We also found that the flicker will hinder the video experience according to our user study. It is also an issue that it is not possible to take into account temporal changes, and predictive generation of objects that frame in / frame out cannot be generated in our model.


% Apply inpainting techniques to this area?
% Test other projection method
% Weighted loss,
% There are a lot of future work to do.


% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
% \begin{figure}[htb]

% \begin{minipage}[b]{1.0\linewidth}
%   \centering
%   \centerline{\includegraphics[width=8.5cm]{image1}}
% %  \vspace{2.0cm}
%   \centerline{(a) Result 1}\medskip
% \end{minipage}
% %
% \begin{minipage}[b]{.48\linewidth}
%   \centering
%   \centerline{\includegraphics[width=4.0cm]{image3}}
% %  \vspace{1.5cm}
%   \centerline{(b) Results 3}\medskip
% \end{minipage}
% \hfill
% \begin{minipage}[b]{0.48\linewidth}
%   \centering
%   \centerline{\includegraphics[width=4.0cm]{image4}}
% %  \vspace{1.5cm}
%   \centerline{(c) Result 4}\medskip
% \end{minipage}
% %
% \caption{Example of placing a figure with experimental results.}
% \label{fig:res}
% %
% \end{figure}


% To start a new column (but not a new page) and help balance the last-page
% column length use \vfill\pagebreak.
% -------------------------------------------------------------------------
%\vfill
%\pagebreak

% \section{REFERENCES}
% \label{sec:ref}

% References should be produced using the bibtex program from suitable
% BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% style file from IEEE produces unsorted bibliography list.
% -------------------------------------------------------------------------

